Noise2Map: End-to-End Diffusion Model for Semantic Segmentation and Change Detection

Semantic segmentation and change detection are two fundamental challenges in remote sensing, requiring models to capture either spatial semantics or temporal differences from satellite imagery. Existing deep learning models often struggle with temporal inconsistencies or in capturing fine-grained spatial structures, require extensive pretraining, and offer limited interpretability - especially in real-world remote sensing scenarios. Recent advances in diffusion models show that Gaussian noise can be systematically leveraged to learn expressive data representations through denoising. Motivated by this, we investigate whether the noise process in diffusion models can be effectively utilized for discriminative tasks. We propose Noise2Map, a unified diffusion-based framework that repurposes the denoising process for fast, end-to-end discriminative learning. Unlike prior work that uses diffusion only for generation or feature extraction, Noise2Map directly predicts semantic or change maps using task-specific noise schedules and timestep conditioning, avoiding the costly sampling procedures of traditional diffusion models. The model is pretrained via self-supervised denoising and fine-tuned with supervision, enabling both interpretability and robustness. Our architecture supports both tasks (SS and CD) through a shared backbone and task-specific noise schedulers. Extensive evaluations on the SpaceNet7, WHU, and xView2 buildings damaged by wildfires datasets demonstrate that Noise2Map ranks on average 1st among seven models on semantic segmentation and 1st on change detection by a cross-dataset rank metric (average F1 primary, IoU tie-break). Ablation studies highlight the robustness of our model against different training noise schedulers and timestep control in the diffusion process, as well as the ability of the model to perform multi-task learning.

==> figure_codes/main_figure.tex <==
\begin{figure}[t]
    \centering
    \resizebox{\columnwidth}{!}{
        \begin{tikzpicture}
            % Row 1 (Semantic Segmentation first)
            \node (seg_img) at (0, 0) {\includegraphics[width=0.1\textwidth]{figures/image_2_input.png}};
            \node[below=0.1cm of seg_img] {Image};

            \node (seg_noisy) at (3, 0) {\includegraphics[width=0.1\textwidth]{figures/Image_A_Step 200.png}};
            \node[below=0.1cm of seg_noisy] {Noisy Image};

            \node (seg_original) at (6, 0) {\includegraphics[width=0.1\textwidth]{figures/image_2_input.png}};
            \node[below=0.1cm of seg_original] {Original Image};

            \node (final_ss) at (9, 0) [draw, minimum width=2cm, minimum height=1.5cm, align=center] {Denoising \\ UNet};
            \node[below=0.1cm of final_ss] {\scriptsize Denoising over timesteps};

            \node (seg_mask) at (12, 0) {\includegraphics[width=0.1\textwidth]{figures/image_2_predicted_mask.png}};
            \node[below=0.1cm of seg_mask] {Segmentation Mask};

            \draw[->, thick] (seg_img.east) -- (seg_noisy.west);
            \draw[->, thick] (seg_noisy.east) -- (seg_original.west);
            \draw[->, thick] (seg_original.east) -- (final_ss.west);
            \draw[->, thick] (final_ss.east) -- (seg_mask.west);

            \draw[decorate,decoration={brace,amplitude=10pt,mirror},thick] 
                (-1, 1) -- (-1, -1) node[midway,right,xshift=0.3cm] {};
            \node at (-2, 0) {SS};

            % Dashed line separating SS and CD
            \draw[dashed, thick] (-1.25, -1.75) -- (13.5, -1.75);

            % Row 2 (Change Detection second)
            \node (img1) at (0, -3) {\includegraphics[width=0.1\textwidth]{figures/Image_A_Original.png}};
            \node[below=0.1cm of img1] {Image 1};

            \node (noisy1) at (3, -3) {\includegraphics[width=0.1\textwidth]{figures/Image_A_Step 200.png}};
            \node[below=0.1cm of noisy1] {Noisy Image 1};

            \node (img2) at (6, -3) {\includegraphics[width=0.1\textwidth]{figures/Image_B_Original.png}};
            \node[below=0.1cm of img2] {Image 2};

            \node (final_cd) at (9, -4.5) [draw, minimum width=2cm, minimum height=1.5cm, align=center] {Denoising \\ UNet};
            \node[below=0.1cm of final_cd] {\scriptsize Denoising over timesteps};

            \node (changemap) at (12, -4.5) {\includegraphics[width=0.1\textwidth]{figures/change_map.png}};
            \node[below=0.1cm of changemap] {Change map};

            \draw[->, thick] (final_cd.east) -- (changemap.west);

            \draw[->, thick] (img1.east) -- (noisy1.west);
            \draw[->, thick] (noisy1.east) -- (img2.west);
            \draw[->, thick] (img2.east) -- ++(0.5, 0) |- (final_cd.west);

            % Second CD row for reversed order
            \node (img2_2) at (0, -6) {\includegraphics[width=0.1\textwidth]{figures/Image_B_Original.png}};
            \node[below=0.1cm of img2_2] {Image 2};

            \node (noisy2) at (3, -6) {\includegraphics[width=0.1\textwidth]{figures/Image_B_Step 200.png}};
            \node[below=0.1cm of noisy2] {Noisy Image 2};

            \node (img1_2) at (6, -6) {\includegraphics[width=0.1\textwidth]{figures/Image_A_Original.png}};
            \node[below=0.1cm of img1_2] {Image 1};

            \draw[->, thick] (img2_2.east) -- (noisy2.west);
            \draw[->, thick] (noisy2.east) -- (img1_2.west);
            \draw[->, thick] (img1_2.east) -- ++(0.5, 0) |- (final_cd.west);

            \draw[decorate,decoration={brace,amplitude=10pt,mirror},thick] 
                (-1, -2) -- (-1, -7) node[midway,right,xshift=0.3cm] {};
            \node at (-2, -4.5) {CD};

        \end{tikzpicture}
    }
    \caption{Illustration of semantic segmentation (SS) and change detection (CD) with noise-driven diffusion process.}
    \label{fig:main_example}
\end{figure}


 % The first two rows demonstrate change detection, and the third row illustrates semantic segmentation with noisy and segmented images. The process begins by adding structured noise to the input, followed by a denoising trajectory that gradually reveals the target output. SHORTER CAPTIONS TO REDUCE TO 9 PAGES AND CHECK TO REMOVE IT

==> figures_and_tables/complexity.tex <==
\iffalse

\begin{table}[ht]
    \centering
    \caption{Model complexity comparison for change detection (CD) and semantic segmentation (SS) tasks. Our proposed \textbf{DDM‑CDSS} supports both tasks. All models are evaluated with 256$\times$256 inputs on a single NVIDIA 3080Ti GPU.}
    \label{tab:complexity}
    \small
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{llcccc}
        \toprule
        \textbf{Task} & \textbf{Model} & \textbf{FLOPs (GMac)} & \textbf{Param (M)} & \textbf{Pretrained On (Size)} & \textbf{Inference Time (ms)} \\
        \midrule
        CD & FCSiamConc       & 18.39       & 43.7   & ImageNet‑1K (1.28M)     & 12.75 \\
        CD & BIT              & 8.74       & 11.94   & ImageNet‑1K (1.28M)     & 19.12 \\
        CD & ChangeFormer‑v6  & 202.96       & 41.03    & ADE20K(25K)/LEVIR‑CD(8.5K)                      & 33.68 \\
        CD & CGNet‑CD         & 87.68       & 38.99   & ImageNet‑1K (1.28M)     & 10.63 \\
        CD & ELGC‑Net         & 188.21       & 10.57   & Scratch                      & 27.99 \\
        CD & DDPM‑CD          & 750       & 437.5  & Sentinel‑2 (500k patches)                      & 490.44 \\
        CD & MambaBCD‑Base    & 44.86       & 92.4   & ImageNet-1K (1.28M)/(LEVIR-CD+, SYSU-CD)                    & 58.76 \\
        \rowcolor{gray!10}
        CD & \textbf{DDM‑CDSS (ours)} & \textbf{248.88} & \textbf{113.7} & \textbf{MajorTom (10K)} & \textbf{36.36} \\
        \arrayrulecolor{gray}\midrule[0.3pt]\arrayrulecolor{black}

        SS & UNet             & 10.74    & 32.5   & ImageNet‑1K (1.28M)     & 7.42 \\
        SS & UNet++           & 57.6     & 48.9   & ImageNet‑1K (1.28M)     & 9.38 \\
        SS & DeepLabV3+       & 9.21     & 26.68   & ImageNet‑1K (1.28M)     & 7.29 \\
        SS & SegFormer        & 2.95      & 5.55    & ImageNet‑1K (1.28M)     & 11.32 \\
        SS & UPerNet          & 19.2     & 37.3   & ImageNet‑1K (1.28M)     & 8.34 \\
        SS & DPT              & 52.07     & 121.0  & ImageNet‑1K (1.28M)     & 12.69 \\
        SS & RS3Mamba         & 11.05       & 43.3   & ImageNet‑1K (1.28M)                      & 40.77 \\
        \rowcolor{gray!10}
        SS & \textbf{DDM‑CDSS (ours)} & \textbf{248.88} & \textbf{113.7} & \textbf{MajorTom (10K Subset)} & \textbf{36.20} \\
        \bottomrule
    \end{tabular}
    }
\end{table}

\fi


\begin{table}[h]
    \centering
    \caption{Model complexity comparison for semantic segmentation (SS) and change detection (CD) tasks. Our proposed \textbf{Noise2Map} supports both tasks. All models are evaluated with 256$\times$256 inputs on a single NVIDIA 3080Ti GPU.}
    \label{tab:complexity}
    \small
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{llccc}
        \toprule
        \textbf{Task} & \textbf{Model} & \textbf{FLOPs (GMac)} & \textbf{Param (M)} & \textbf{Inference Time (ms)} \\
        \midrule
        SS & UNet             & 10.74       & 32.5    & 7.42 \\
        SS & UNet++           & 57.6        & 48.9    & 9.38 \\
        SS & DeepLabV3+       & 9.21        & 26.68   & 7.29 \\
        SS & SegFormer        & 2.95        & 5.55    & 11.32 \\
        SS & UPerNet          & 19.2        & 37.3    & 8.34 \\
        SS & DPT              & 52.07       & 121.0   & 12.69 \\
        SS & RS3Mamba         & 11.05       & 43.3    & 40.77 \\
        \rowcolor{gray!10}
        SS & Noise2Map (ours) & 248.88 & 113.7 & 36.20 \\
        \arrayrulecolor{gray}\midrule[0.3pt]\arrayrulecolor{black}
        
        CD & FCSiamConc       & 18.39       & 43.7    & 12.75 \\
        CD & BIT              & 8.74        & 11.94   & 19.12 \\
        CD & ChangeFormer-v6  & 202.96      & 41.03   & 33.68 \\
        CD & CGNet-CD         & 87.68       & 38.99   & 10.63 \\
        CD & ELGC-Net         & 188.21      & 10.57   & 27.99 \\
        CD & DDPM-CD          & 750         & 437.5   & 490.44 \\
        CD & MambaBCD-Base    & 44.86       & 92.4    & 58.76 \\
        \rowcolor{gray!10}
        CD & Noise2Map (ours) & 248.88 & 113.7 & 36.36 \\
        \bottomrule
    \end{tabular}
    }
\end{table}


==> figures_and_tables/single_vs_multi_task.tex <==
\begin{figure}[h]
  \centering

  % -------- Change Detection (CD) - Sample 1 --------
  \begin{subfigure}{\linewidth}
    \centering
    \begin{subfigure}{0.18\linewidth}
      \centering
      \caption*{\scriptsize Pre-Image}
      \includegraphics[width=\linewidth]{figures/single-multi-task/sample_1/post_image.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.18\linewidth}
      \centering
      \caption*{\scriptsize Post-Image}
      \includegraphics[width=\linewidth]{figures/single-multi-task/sample_1/pre_image.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.18\linewidth}
      \centering
      \caption*{\scriptsize Single-Task}
      \includegraphics[width=\linewidth]{figures/single-multi-task/sample_1/single_task_cd.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.18\linewidth}
      \centering
      \caption*{\scriptsize Multi-Task}
      \includegraphics[width=\linewidth]{figures/single-multi-task/sample_1/multi_task_cd.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.18\linewidth}
      \centering
      \caption*{\scriptsize Ground Truth}
      \includegraphics[width=\linewidth]{figures/single-multi-task/sample_1/true_change_map.png}
    \end{subfigure}
  \end{subfigure}

  \\[0.25em] % Adds spacing between the two rows

  % -------- Change Detection (CD) - Sample 2 --------
  \begin{subfigure}{\linewidth}
    \centering
    \begin{subfigure}{0.18\linewidth}
      \centering
      % \caption*{\scriptsize Pre-Image}
      \includegraphics[width=\linewidth]{figures/single-multi-task/sample_2/post_image.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.18\linewidth}
      \centering
      % \caption*{\scriptsize Post-Image}
      \includegraphics[width=\linewidth]{figures/single-multi-task/sample_2/pre_image.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.18\linewidth}
      \centering
      % \caption*{\scriptsize Single-Task}
      \includegraphics[width=\linewidth]{figures/single-multi-task/sample_2/single_task_cd.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.18\linewidth}
      \centering
      % \caption*{\scriptsize Multi-Task}
      \includegraphics[width=\linewidth]{figures/single-multi-task/sample_2/multi_task_cd.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.18\linewidth}
      \centering
      % \caption*{\scriptsize Ground Truth}
      \includegraphics[width=\linewidth]{figures/single-multi-task/sample_2/true_change_map.png}
    \end{subfigure}
    \caption{CD: Multi-task improves CD alignment with ground truth}
  \end{subfigure}

  % \\[0.25em] % Adds spacing between the two rows

  % -------- Semantic Segmentation (SS) - Sample 1 --------
  \begin{subfigure}{\linewidth}
    \centering
    \begin{subfigure}{0.18\linewidth}
      \centering
      \caption*{\scriptsize Input Image}
      \includegraphics[width=\linewidth]{figures/single-multi-task/sample_1/ss_input.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.18\linewidth}
      \centering
      \caption*{\scriptsize Single-Task}
      \includegraphics[width=\linewidth]{figures/single-multi-task/sample_1/single_task_ss.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.18\linewidth}
      \centering
      \caption*{\scriptsize Multi-Task}
      \includegraphics[width=\linewidth]{figures/single-multi-task/sample_1/multi_task_ss.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.18\linewidth}
      \centering
      \caption*{\scriptsize Ground Truth}
      \includegraphics[width=\linewidth]{figures/single-multi-task/sample_1/true_ss_mask.png}
    \end{subfigure}
  \end{subfigure}

  \\[0.25em] % Adds spacing between the two rows

  % -------- Semantic Segmentation (SS) - Sample 2 --------
  \begin{subfigure}{\linewidth}
    \centering
    \begin{subfigure}{0.18\linewidth}
      \centering
      % \caption*{\scriptsize Input Image}
      \includegraphics[width=\linewidth]{figures/single-multi-task/sample_2/ss_input.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.18\linewidth}
      \centering
      % \caption*{\scriptsize Single-Task}
      \includegraphics[width=\linewidth]{figures/single-multi-task/sample_2/single_task_ss.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.18\linewidth}
      \centering
      % \caption*{\scriptsize Multi-Task}
      \includegraphics[width=\linewidth]{figures/single-multi-task/sample_2/multi_task_ss.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.18\linewidth}
      \centering
      % \caption*{\scriptsize Ground Truth}
      \includegraphics[width=\linewidth]{figures/single-multi-task/sample_2/true_ss_mask.png}
    \end{subfigure}
    \caption{SS: Single-task improves SS alignment with ground truth}
  \end{subfigure}

  \caption{Single-Task vs. Multi-Task Learning Setup: (a) Change Detection (CD) and (b) Semantic Segmentation (SS)}
  
  \vspace{-0.5mm}
  \label{fig:cd_ss_comparison}
\end{figure}


==> sections/5_limitations.tex <==
% If Any

